What's Pulling the Strings? Evaluating Integrity and Attribution in AI Training and Inference through Concept Shift

The growing adoption of artificial intelligence (AI) has amplified concerns about trustworthiness, including integrity, privacy, robustness, and bias. To assess and attribute these threats, we propose ConceptLens, a generic framework that leverages pre-trained multimodal models to identify the root causes of integrity threats by analyzing Concept Shift in probing samples. ConceptLens demonstrates strong detection performance for vanilla data poisoning attacks and uncovers vulnerabilities to bias injection, such as the generation of covert advertisements through malicious concept shifts. It identifies privacy risks in unaltered but high-risk samples, filters them before training, and provides insights into model weaknesses arising from incomplete or imbalanced training data. Additionally, at the model level, it attributes concepts that the target model is overly dependent on, identifies misleading concepts, and explains how disrupting key concepts negatively impacts the model. Furthermore, it uncovers sociological biases in generative content, revealing disparities across sociological contexts. Strikingly, ConceptLens reveals how safe training and inference data can be unintentionally and easily exploited, potentially undermining safety alignment. Our study informs actionable insights to breed trust in AI systems, thereby speeding adoption and driving greater innovation.

==> tables/brand.tex <==
\begin{table*}[t]
\centering
\caption{Advertisement generation rate for open source models. Here, we only counted the generated samples that contain clearly recognizable brand logo. }
\resizebox{\linewidth}{!}{%
\scriptsize
\begin{tabular}{llcccccccccccccccccc}
\toprule
\textbf{Type} & \textbf{Item} & \multicolumn{3}{c}{\textbf{Stable Diffusion 1.4 (n=160)}} & \multicolumn{3}{c}{\textbf{Stable Diffusion 2.1 (n=160)}} & \multicolumn{3}{c}{\textbf{Stable Diffusion XL (n=160)}} & \multicolumn{3}{c}{\textbf{Stable Diffusion 3 (n=160)}} & \multicolumn{3}{c}{\textbf{Flux-1 (n=160)}} \\
 &  & op & op+b & op-b & op & op+b & op-b & op & op+b & op-b & op & op+b & op-b & op & op+b & op-b \\
\midrule
Packaged Food & Cola & 0.094 & 0.119 & 0.038 & 0.000 & 0.006 & 0.000 & \cellcolor{red!50}0.406 & \cellcolor{red!50}0.438 & 0.206 & \cellcolor{red!50}0.738 & 0.031 & 0.000 & \cellcolor{red!50}0.594 & \cellcolor{red!50}0.600 & \cellcolor{red!50}0.488 \\
Packaged Food & Energy drink & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
Packaged Food & Potato Chips & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor{red!50} 0.331 & 0.031 \\
Electronic device & smartphone & 0.000 & 0.000 & 0.006 & 0.000 & 0.000 & 0.000 & 0.019 & 0.013 & 0.019 & 0.013 & 0.019 & 0.019 & 0.075 & 0.138 & 0.050 \\
Electronic device & laptop & 0.013 & 0.031 & 0.081 & 0.006 & 0.038 & 0.063 & 0.063 & 0.125 & 0.019 & 0.119 & \cellcolor{red!50}0.669 & \cellcolor{red!50}0.594 & 0.244 & 0.219 & \cellcolor{red!50}0.594 \\
Electronic device & tablet & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.019 & 0.031 & 0.006 \\
Fashion & Monogram Bag & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.250 & 0.238 & \cellcolor{red!50}0.963 & \cellcolor{red!50}0.925 & \cellcolor{red!50}1.000 \\
Fashion & Wallet & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
Fast food & Fries & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
Luxury car & Sedan & 0.000 & 0.019 & 0.006 & 0.000 & 0.019 & 0.025 & 0.000 & 0.000 & 0.050 & 0.000 & 0.000 & 0.000 & 0.119 & 0.025 & 0.069 \\
Luxury car & Suv & 0.025 & 0.031 & 0.013 & 0.013 & 0.031 & 0.063 & 0.131 & 0.200 & 0.100 & 0.000 & \cellcolor{red!50}0.350 & 0.225 & \cellcolor{red!50}0.350 & 0.200 & 0.225 \\
Luxury car & Electric Car & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
Luxury car & MPV & 0.000 & 0.000 & 0.006 & 0.000 & 0.019 & 0.013 & 0.000 & 0.000 & 0.075 & 0.006 & 0.275 & 0.125 & 0.125 & 0.275 & 0.125 \\
% Repeat the structure for other rows and datasets
% Highlight cells with values > 0.3 using \cellcolor{red!50}
\bottomrule
\end{tabular}
}
\begin{tablenotes}
\item[]op: original prompt in Appendix~\ref{sec:prompt}; op + b: original prompt + ``with brand''; op + b: original prompt + ``without brand''.
\end{tablenotes}
\label{tab:brand_open_sourse}
\end{table*}



\begin{table}[t]
\centering
\caption{Advertisement generation rate for closed source models. Here, we only counted the generated samples that contain clearly recognizable brand logo.}

\resizebox{\linewidth}{!}{
\begin{tabular}{llccccccccccccccc}
\toprule
\textbf{Type} & \textbf{Item} & \multicolumn{3}{c}{\textbf{Dalle 2 (n=20)}} & \multicolumn{3}{c}{\textbf{Dalle 3 (n=20)}} & \multicolumn{3}{c}{\textbf{Midjourney (n=20)}} & \multicolumn{3}{c}{\textbf{TongYiWangXiang (n=20)}} \\
 &  & op & op+b & op-b & op & op+b & op-b & op & op+b & op-b & op & op+b & op-b \\
\midrule
Packaged Food & Cola & 0.000 & 0.000 & 0.000 & 0.200 & 0.250 & \cellcolor{red!50}0.350 & \cellcolor{red!50}0.350 & \cellcolor{red!50}0.550 & 0.300 & \cellcolor{red!50}0.700 & \cellcolor{red!50}0.900 & \cellcolor{red!50}0.850 \\
Packaged Food & Energy drink & 0.000 & 0.000 & 0.000 & 0.050 & 0.200 & 0.000 & 0.000 & 0.100 & 0.000 & 0.050 & 0.300 & 0.150 \\
Packaged Food & Potato Chips & 0.000 & 0.000 & 0.000 & \cellcolor{red!50}0.400 & \cellcolor{red!50}0.450 & 0.200 & 0.000 & 0.000 & 0.000 & 0.100 & \cellcolor{red!50}0.800 & \cellcolor{red!50}0.450 \\
Electronic device & smartphone & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.050 & 0.250 & 0.000 & 0.050 & 0.050 & 0.000 \\
Electronic device & laptop & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor{red!50}0.850 & \cellcolor{red!50}0.950 & \cellcolor{red!50}0.550 & 0.200 & \cellcolor{red!50}0.700 & \cellcolor{red!50}0.350 \\
Electronic device & tablet & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.050 & \cellcolor{red!50}0.350 & 0.000 & 0.150 & \cellcolor{red!50}0.350 & 0.200 \\
Fashion & Monogram Bag & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor{red!50}0.500 & \cellcolor{red!50}0.800 & \cellcolor{red!50}0.900 \\
Fashion & Wallet & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.100 & \cellcolor{red!50}0.400 & 0.300 \\
Fast food & Fries & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.100 & \cellcolor{red!50}0.700 & \cellcolor{red!50}0.450 \\
Luxury car & Sedan & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.100 & \cellcolor{red!50}0.350 & 0.000 & 0.000 & 0.000 & 0.000 \\
Luxury car & Suv & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.300 & 0.250 & 0.100 & 0.000 & 0.000 & 0.000 \\
Luxury car & Electric Car & 0.000 & 0.000 & 0.000 & 0.000 & 0.050 & 0.000 & 0.100 & 0.150 & 0.050 & 0.100 & 0.150 & 0.150 \\
Luxury car & MPV & 0.000 & 0.000 & 0.000 & 0.000 & 0.050 & 0.000 & 0.150 & 0.050 & 0.000 & 0.000 & 0.000 & 0.000 \\
\bottomrule
\end{tabular}
}

\label{tab:brand_close_sourse}
\begin{tablenotes}
\item[]op: original prompt in Appendix~\ref{sec:prompt}; op + b: original prompt + ``with brand''; op + b: original prompt + ``without brand''.
\end{tablenotes}
\end{table}

==> tables/detection_multi_VGVE.tex <==
% \begin{table}[t]
% \caption{Adversarial attack detection performance on ALBEF for VG task with RefCOCO+ and VE task with SNLI-VE. DR and FPR is respectively the Detection Rate and False Positive Rate of a given detection method.
% }
% \label{tab:detection_multi_VGVE}
% \centering
% \resizebox{\linewidth}{!}{%
% \setlength{\aboverulesep}{0pt}
% \setlength{\belowrulesep}{0pt}
% \setlength{\extrarowheight}{.75ex}
% \begin{tabular}{lccccccc>{\columncolor[gray]{0.85}}c>{\columncolor[gray]{0.85}}c}
% \toprule
% \multicolumn{2}{c}{Attack Setting} & \multicolumn{6}{c}{Detection Baseline} & \multicolumn{2}{c}{\textbf{\sol{} (Ours)}} \\ 
% \midrule
% \multirow{2}{*}{VLP task}   & \multirow{2}{*}{Attack type} & \multicolumn{2}{c}{Z-score\cite{meng2017magnet}} & \multicolumn{2}{c}{PPL~\cite{alon2023detecting} }   & \multicolumn{2}{c}{MPL}  & \multicolumn{2}{c}{Elliptic Envelope~\cite{0d23955b-2c3d-3692-b621-b91e68c0944a}} \\ 
%  \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10}
%                 &   & DR       & FPR      & DR       & FPR  &DR & FPR&DR & FPR \\ \midrule
% \multirow{5}{*}{VG}   & Bert-attack   &0.2&0.15& 0.2&0.15&0.73&0.10& \textbf{0.855}    & \textbf{0.01}   \\ 
% % \cmidrule{2-16} 
%                         & PGD-attack  & 0.17&  0.17   &  0.18    & 0.15 &0.15& 0.15 & \textbf{0.81 } & \textbf{0.015}    \\ 
% % \cmidrule{2-16} 
%                         & Sep-attack  &0.22&0.18&0.18& 0.15    &    0.70  &0.10   & \textbf{0.935 } &\textbf{ 0.01}   \\ 
%                         & Co-attack  &0.24&0.19&0.215 &0.15     &   0.69   & 0.125     & \textbf{0.925 }   &\textbf{ 0.01}   \\  
                        
% \midrule 

% \multirow{5}{*}{VE}   & Bert-attack   &0.14&0.13&0.18 &0.15&0.81&0.15& \textbf{ 0.94}    & \textbf{0.01 }  \\ 
% % \cmidrule{2-16} 
%                         & PGD-attack  &0.15&0.16&0.15 &0.15     &     0.18 & 0.18  & \textbf{0.71 }  & \textbf{0.01 }   \\ 
% % \cmidrule{2-16} 
%                         & Sep-attack  &0.14&0.14&0.15 &0.15     &0.82      & 0.18  & \textbf{0.99}    & \textbf{0.015}   \\ 
%                         & Co-attack  &0.15&0.17&0.16 &0.15     &0.69      &0.14      & \textbf{0.985 }   & \textbf{0.015}   \\ 
                        
% \bottomrule
% \end{tabular}
% }
% \end{table}

